On $r$-Simple $k$-Path and Related Problems Parameterized by $k/r$

Abasi et al. (2014) and Gabizon et al. (2015) studied the following problems. In the $r$-Simple $k$-Path problem, given a digraph $G$ on $n$ vertices and integers $r,k$, decide whether $G$ has an $r$-simple $k$-path, which is a walk where every vertex occurs at most $r$ times and the total number of vertex occurrences is $k$. In the $(r,k)$-Monomial Detection problem, given an arithmetic circuit that encodes some polynomial $P$ on $n$ variables and integers $k,r$, decide whether $P$ has a monomial of degree $k$ where the degree of each variable is at most~$r$. In the $p$-Set $(r,q)$-Packing problem, given a universe $V$, positive integers $p,q,r$, and a collection $\cal H$ of sets of size $p$ whose elements belong to $V$, decide whether there exists a subcollection ${\cal H}'$ of $\cal H$ of size $q$ where each element occurs in at most $r$ sets of ${\cal H}'$. Abasi et al. and Gabizon et al. proved that the three problems are single-exponentially fixed-parameter tractable (FPT) when parameterized by $(k/r)\log r$, where $k=pq$ for $p$-Set $(r,q)$-Packing and asked whether the $\log r$ factor in the exponent can be avoided. We consider their question from a wider perspective: are the above problems FPT when parameterized by $k/r$ only? We resolve the wider question by (a) obtaining a $2^{O((k/r)^2\log(k/r))} (n+\log k)^{O(1)}$-time algorithm for $r$-Simple $k$-Path on digraphs and a $2^{O(k/r)} (n+\log k)^{O(1)}$-time algorithm for $r$-Simple $k$-Path on undirected graphs (i.e., for undirected graphs we answer the original question in affirmative), (b) showing that $p$-Set $(r,q)$-Packing is FPT, and (c) proving that $(r,k)$-Monomial Detection is para-NP-hard. For $p$-Set $(r,q)$-Packing, we obtain a polynomial kernel for any fixed $p$, which resolves a question posed by Gabizon et al. regarding the existence of polynomial kernels for problems with relaxed disjointness constraints.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-authordraft.tex \
	samples/sample-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-acmsmall.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmsmall]{acmart}/' $< > $@

samples/sample-acmlarge.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmlarge,screen]{acmart}/' $< > $@

samples/sample-acmtog.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmtog]{acmart}/' $<   > $@

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-authordraft.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf,authordraft]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-xelatex.tex: samples/sample-sigconf.tex
	cp $< $@

samples/sample-sigplan.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigplan,screen]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi-a.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi-a]{acmart}/' $< | \
	sed 's/begin{figure}\[h\]/begin{marginfigure}/' | \
	sed 's/end{figure}/end{marginfigure}/' | \
	sed 's/begin{table}/begin{margintable}/' | \
	sed 's/end{table}/end{margintable}/'   > $@


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> UndirectedPseudocode.tex <==
%!TEX root = Main-Repetitions.tex

\section{Pseudocode of the Algorithm}\label{sec:pseudocode}

Given that our algorithm for {\sc Undirected $r$-Simple $k$-Path} is optimal under the ETH, we present its pseudocode (in Algorithm \ref{undirectedPseuodo}) in case it is to be implemented. The pseudocode uses the algorithm in Lemma \ref{lem:tw2CompDP} as a black box. The precise details of the implementation of this black box are explicitly given in the beginning of the proof of Lemma \ref{lem:tw2CompDP}.


\begin{algorithm}
\caption{Algorithm for {\sc Undirected $r$-Simple $k$-Path}}\label{undirectedPseuodo}
\begin{algorithmic}[1]
\If{$r\leq\sqrt{k}$}
	\State Use Algorithm \ref{undirectedPseuodo1} to solve the input instance
\Else
	\State Use Algorithm \ref{undirectedPseuodo2} to solve the input instance
\EndIf
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Algorithm for {\sc Undirected $r$-Simple $k$-Path}: Case 1 ($r\leq \sqrt{k}$)}\label{undirectedPseuodo1}
\begin{algorithmic}[1]
	\ForAll{$\mathsf{col}\in{\cal F}$, $\overline{\bf d}\in {\cal D}_{k,r}$}
		\State Color $G$ by $\mathsf{col}$
		\State Allocate $\mathsf{N}$ with an entry $[v,\overline{\bf d}',C]$ for all $v\in V(G)$, $\overline{\bf d}'=(d'_1,\ldots,d'_{\mathsf{b}(k/r)})\in{\cal D}_{r,k}$ such that $d_i'\in\{0,\ldots,d_i\}$ for all $i\in\{1,\ldots,\mathsf{b}(k/r)\}$, and $C\subseteq\{1,\ldots,\mathsf{b}(k/r)\}$
		\State Initialize all $\mathsf{N}[v,\overline{\bf d}',C]$ where $\sum_{i=1}^{\mathsf{b}(k/r)}d'_i\leq 1$: if $d_{\mathsf{col}(v)}'\neq 1$, then $\mathsf{N}[v,\overline{\bf d}',C]=-\infty$; otherwise, $\mathsf{N}[v,\overline{\bf d}',C]$ is the maximum of $0$ and the output of algorithm in Lemma \ref{lem:tw2CompDP} with input $(G,C,v,\overline{\bf d})$
		\ForAll{$\mathsf{N}[v,\overline{\bf d}',C]$ in increasing order on $\sum_{i=1}^{\mathsf{b}(k/r)}d'_i\geq 2$}
			\If{$d'_{\mathsf{col(v)}}=0$}		
				\State $\mathsf{N}[v,\overline{\bf d}',C]=-\infty$
			\Else
				\State Let $\overline{\bf d}''=(d''_1,\ldots,d''_{\mathsf{b}(k/r)})$ where $d''_{\mathsf{col(v)}}=d'_{\mathsf{col(v)}}-1$ and $d''_i=d'_i$ for all $i\in\{1,\ldots,\mathsf{b}(k/r)\}\setminus\{\mathsf{col}(v)\}$
				\ForAll{$C'\subseteq C$}
					\State Let $A_{C'}$ be the output of algorithm in Lemma \ref{lem:tw2CompDP} with input $(G,C',v,\overline{\bf d})$
				\EndFor
				\State $\displaystyle{\mathsf{N}[v,\overline{\bf d}',C]=\max_{u:\{u,v\}\in E(G)}\left(\max\left\{1+\mathsf{N}[u,\overline{\bf d}'',C],\max_{C'\subseteq C}(A_{C'}+1+\mathsf{N}[u,\overline{\bf d}'',C\setminus C'])\right\}\right)}$
			\EndIf
		\EndFor
		\ForAll{$\mathsf{N}[v,\overline{\bf d}',C]$ with $\overline{\bf d}'=\overline{\bf d}$}
			\If{$\mathsf{N}[v,\overline{\bf d}',C]\geq k-1$}
				\Return "Yes-instance"
			\EndIf
		\EndFor
	\EndFor
	\Return "No-instance"
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Algorithm for {\sc Undirected $r$-Simple $k$-Path}: Case 2 ($r>\sqrt{k}$)}\label{undirectedPseuodo2}
\begin{algorithmic}[1]
	\State Compute a maximal matching $M$ in $G$
	\State Let $U$ be the set of endpoints of edges in $M$
	\If{$|U|>3k/r$}
		\Return "Yes-instance"
	\Else
		\ForAll{$U'\subseteq U$, $\mathsf{col}\in{\cal F}$, $\overline{\bf d}\in {\cal D}_{k,r}$ with $d_{\mathsf{col(v)}}\geq 1$ for all $v\in U'$}\label{step:loop}
			\State Color $G$ by $\mathsf{col}$
			\State Let $G'=G-X$ for $X=(U\setminus U')\cup\{v\in V(G)\setminus U: $ there exists a vertex in $U'$ with the same color as $v\}$			
			\State Allocate $\mathsf{N}$ with an entry $[v,\overline{\bf d}']$ for all $v\in V(G')$, and $\overline{\bf d}'=(d'_1,\ldots,d'_{\mathsf{b}(k/r)})\in{\cal D}_{r,k}$ such that $d_i'\in\{0,\ldots,d_i\}$ for all $i\in\{1,\ldots,\mathsf{b}(k/r)\}$
		\State Initialize all $\mathsf{N}[v,\overline{\bf d}']$ where $\sum_{i=1}^{\mathsf{b}(k/r)}d'_i\leq 1$: if $d_{\mathsf{col}(v)}'\neq 1$, then $\mathsf{N}[v,\overline{\bf d}']=\mathsf{false}$; otherwise, $\mathsf{N}[v,\overline{\bf d}']=\mathsf{true}$
		\ForAll{$\mathsf{N}[v,\overline{\bf d}']$ in increasing order on $\sum_{i=1}^{\mathsf{b}(k/r)}d'_i\geq 2$}
			\If{$d'_{\mathsf{col(v)}}=0$}		
				\State $\mathsf{N}[v,\overline{\bf d}']=\mathsf{false}$
			\Else
				\State Let $\overline{\bf d}''=(d''_1,\ldots,d''_{\mathsf{b}(k/r)})$ where $d''_{\mathsf{col(v)}}=d'_{\mathsf{col(v)}}-1$ and $d''_i=d'_i$ for all $i\in\{1,\ldots,\mathsf{b}(k/r)\}\setminus\{\mathsf{col}(v)\}$
				\State $\displaystyle{\mathsf{N}[v,\overline{\bf d}']=\mathsf{OR}_{u:\{u,v\}\in E(G')}(1+\mathsf{N}[u,\overline{\bf d}''])}$
			\EndIf
		\EndFor
		\If{$\mathsf{OR}_{v\in V(G')}\mathsf{N}[v,\overline{\bf d}]=\mathsf{false}$}
			\State Go to Step \ref{step:loop}
		\EndIf			
			
		\State Let $c_v=r-d_{\mathsf{col(v)}}$ for all $v\in V(G')$,  $F=\sum_{v\in V(G')}c_v$ and $\ell=2(k-\sum_{i=1}^{\mathsf{b}(k/r)}d_i)$
		\State Construct a flow network $N$ with source $s$ and sink $t$ as follows.  For all $v\in V(G')$, insert (into $N$) two new vertices, $v_1$ and $v_2$, the arc $(v_1,v_2)$ of infinite (upper) capacity and cost $1$, and the arcs $(s,v_1)$ and $(v_2,t)$ both of (upper) capacity $c_v$ and cost $0$.  For all $\{u,v\}\in E(G')$, insert (into $N$) the arcs $(u_1,v_2)$ and $(v_1,u_2)$ both of infinite (upper) capacity and cost $0$.
		\State Compute the minimum cost $C$ required to send $F$ units of (integral) flow from $s$ to $t$ in $N$ in polynomial time
		\If{$C\leq F-\ell$}
			\Return "Yes-instance"
		\EndIf					
		\EndFor		
		\Return "No-instance"
	\EndIf
\end{algorithmic}
\end{algorithm}

